Photoelectron Spectroscopy and Circular Dichroism of an Open-Shell Organometallic Camphor Complex

We present an investigation of one-photon valence-shell photoelectron spectroscopy and photoelectron circular dichroism (PECD) for the chiral molecule (1R,4R)-3-(heptafluorobutyryl)-(+)-camphor (HFC) and its europium complex Eu(III) tris[3-(heptafluorobutyryl)-(1R,4R)-camphorate] (Eu-HFC$_{3}$), the latter of which constitutes the heaviest organometallic molecule for which PECD has yet been measured. We discuss the role of keto-enol tautomerism in HFC, both as a free molecule and complexed in Eu-HFC$_{3}$. PECD is a uniquely sensitive probe of molecular chirality and structure such as absolute configuration, conformation, isomerisation, and substitution, and as such is in principle well suited to unambiguously resolving tautomers; however modeling remains challenging. For small organic molecules, theory is generally capable of accounting for experimentally measured PECD asymmetries, but significantly poorer agreement is typically achieved for the case of large open-shell systems. Here, we report PECD asymmetries ranging up to $\sim8\%$ for HFC and $\sim7\%$ for Eu-HFC$_{3}$, of similar magnitude to those reported previously for smaller isolated chiral molecules, indicating that PECD remains a practical experimental technique for the study of large, complicated chiral systems.

==> xx.tex <==



==> xx2.tex <==


